Distantly-Supervised Evidence Retrieval Enables Question Answering without Evidence Annotation

Open-domain question answering answers a question based on evidence retrieved from a large corpus. State-of-the-art neural approaches require intermediate evidence annotations for training. However, such intermediate annotations are expensive, and methods that rely on them cannot transfer to the more common setting, where only question-answer pairs are available. This paper investigates whether models can learn to find evidence from a large corpus, with only distant supervision from answer labels for model training, thereby generating no additional annotation cost. We introduce a novel approach (DistDR) that iteratively improves over a weak retriever by alternately finding evidence from the up-to-date model and encouraging the model to learn the most likely evidence. Without using any evidence labels, DistDR is on par with fully-supervised state-of-the-art methods on both multi-hop and single-hop QA benchmarks. Our analysis confirms that DistDR finds more accurate evidence over iterations, which leads to model improvements.

==> 2021_emnlp_weak_dpr/tables/human-eval.tex <==

\begin{table}[!tb]
    \centering
    \small
      \begin{tabular}{lc}
        \toprule
         \textbf{Category}  & \textbf{$\%$}\\
       \midrule
       Answerable via single evidence & 38  \\
       Alternate evidence & 28  \\
        Wrong evidence & 34  \\
      \bottomrule
      \end{tabular}
      \caption{We manually analyze 50 questions on \hotpot{} training set where the retrieved evidence is unlike the annoated evidence. 
      }
    \label{tb:human-eval}

  \end{table}


==> scripts/git-latexdiff <==
#! /bin/bash

# Main author: Matthieu Moy <Matthieu.Moy@imag.fr> (2012 - 2016)
# (See the Git history for other contributors)
#
# Copying and distribution of this file, with or without modification,
# are permitted in any medium without royalty provided the copyright
# notice and this notice are preserved.  This file is offered as-is,
# without any warranty.
#
# git-latexdiff is a wrapper around latexdiff
# (http://www.ctan.org/pkg/latexdiff) that allows using it to diff two
# revisions of a LaTeX file.
#
# The script internally checks out the full tree for the specified
# revisions, calls latexpand to flatten the document and then calls
# latexdiff, hence this works if the document is split into multiple
# .tex files.
#
# Try "git latexdiff -h" for more information.
#
# To install, just copy git-latexdiff in your $PATH.

# Missing features (patches welcome ;-):
# - diff the index
# - hardlink temporary checkouts as much as possible

# Alternatives:
#
# There is another script doing essentially the same here:
# https://github.com/cawka/latexdiff/blob/master/latexdiff-git
# My experience is that latexdiff-git is more buggy than
# git-latexdiff, but they probably just don't have the same bugs ;-)
#
# There are a bunch of other alternatives cited here:
#
#   http://tex.stackexchange.com/questions/1325/using-latexdiff-with-git
#
# Ideally, these scripts should be merged.

set -o errexit
set -o noclobber

# Some versions of git set $GIT_WORK_TREE when ran through an alias.
# This wouldn't work with git-latexdiff which plays with different
# work trees.
unset GIT_DIR
unset GIT_WORK_TREE

# (Comment and 'unset' line borrowed from Git's source code)
# Having this variable in your environment would break scripts because
# you would cause "cd" to be taken to unexpected places.  If you
# like CDPATH, define it for your interactive shell sessions without
# exporting it.
# But we protect ourselves from such a user mistake nevertheless.
unset CDPATH

# @GIT_LATEXDIFF_VERSION@ is substituted by the install script here,
# but not within git_latexdiff_compute_version().
git_latexdiff_version='@GIT_LATEXDIFF_VERSION@'

git_latexdiff_compute_version () {
    if [ "$git_latexdiff_version" = '@GIT_LATEXDIFF''_VERSION@' ]; then
	(cd "$(dirname "$0")" && git describe --tags HEAD 2>/dev/null || echo 'Unknown version')
    else
	echo "$git_latexdiff_version"
    fi
}

usage () {
    cat << EOF
Usage: $(basename "$0") [options] OLD [NEW]
       $(basename "$0") [options] OLD --
       $(basename "$0") [options] -- OLD
Call latexdiff on two Git revisions of a file.

OLD and NEW are Git revision identifiers. NEW defaults to HEAD.
If "--" is used for NEW, then diff against the working directory.

Options:
    --help                this help message
    --main <file.tex>     name of the main LaTeX file
    --no-view             don't display the resulting PDF file
    --latex               run latex instead of pdflatex
    --bibtex, -b          run bibtex as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --biber               run BibLaTex-Biber as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --view                view the resulting PDF file
                            (default if -o is not used)
    --pdf-viewer <cmd>    use <cmd> to view the PDF file (default: \$PDFVIEWER)
    --no-cleanup          don't cleanup temp dir after running
    --no-flatten          don't call latexpand to flatten the document
    --cleanup MODE        Cleanup temporary files according to MODE:

                           - keeppdf (default): keep only the
                                  generated PDF file

                           - none: keep all temporary files
                                  (may eat your diskspace)

                           - all: erase all generated files.
                                  Problematic with --view when the
                                  viewer is e.g. evince, and doesn't
                                  like when the file being viewed is
                                  deleted.

    --latexmk             use latexmk
    --latexopt            pass additional options to latex (e.g. -shell-escape)
    -o <file>, --output <file>
                          copy resulting PDF into <file> (usually ending with .pdf)
                          Implies "--cleanup all"
    --tmpdirprefix        where temporary directory will be created (default: /tmp)
    --verbose, -v         give more verbose output
    --quiet               redirect output from subprocesses to log files
    --prepare <cmd>       run <cmd> before latexdiff (e.g. run make to generate
                             included files)
    --ln-untracked        symlink uncommited files from the working directory
    --version             show git-latexdiff version.
    --subtree             checkout the tree at and below the main file
                             (enabled by default, disable with --whole-tree)
    --whole-tree          checkout the whole tree (contrast with --subtree)
    --ignore-latex-errors keep on going even if latex gives errors, so long as
                          a PDF file is produced
    --ignore-makefile     ignore the Makefile, build as though it doesn't exist
    -*                    other options are passed directly to latexdiff
    --bbl                 shortcut to flatten a bbl file of the same name as the project
    --latexpand           pass options to latexpand (should be last option specified)
    --latexdiff-flatten   use --flatten from latexdiff instead of latexpand
EOF
}

die () {
    echo "fatal: $*"
    exit 1
}

verbose () {
    if test "$verbose" = 1 ; then
	printf "%s ..." "$@"
    fi
}

verbose_progress () {
    if test "$verbose" = 1 ; then
	printf "."
    fi
}

verbose_done () {
    if test "$verbose" = 1 ; then
	echo " ${1:-done}."
    fi
}

verbose_say () {
    if test "$verbose" = 1 ; then
	printf "%s\n" "$@"
    fi
}

old=
new=
main=
view=maybe
cleanup=keeppdf
verbose=0
bibtex=0
biber=0
output=
initial_dir=$PWD
initial_repo=$(git rev-parse --show-toplevel)
tmpdir_prefix="/tmp"
prepare_cmd=
flatten=1
subtree=1
uselatexmk=
latexopt=
ln_untracked=0
quiet=0
ignorelatexerrors=0
latexdiffopt=()
latexpand=()
bbl=0
latexdiff_flatten=0
latex=0


while test $# -ne 0; do
    case "$1" in
        "--help"|"-h")
            usage
            exit 0
            ;;
	"--main")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    main=$1
	    ;;
	"--no-view")
	    view=0
	    ;;
	"--view")
	    view=1
	    ;;
	"--pdf-viewer")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    PDFVIEWER="$1"
	    ;;
	"--no-cleanup")
	    cleanup=none
	    ;;
	"--ignore-latex-errors")
	    ignorelatexerrors=1
	    ;;
        "--cleanup")
            shift
            case "$1" in
                "none"|"all"|"keeppdf")
                    cleanup="$1"
                    ;;
                *)
                    echo "Bad argument --cleanup $1"
                    usage
                    exit 1
                    ;;
            esac
            ;;
	"--no-flatten")
            flatten=0
            ;;
	"--ignore-makefile")
	    ignoremake=1
	    ;;
	"-o"|"--output")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    output=$1
	    cleanup=all
	    ;;
	"-b"|"--bibtex")
	    bibtex=1
	    ;;
	"--latex")
	    latex=1
	    ;;
	"--biber")
	    biber=1
	    ;;
	"--verbose"|"-v")
	    verbose=1
	    ;;
        "--quiet")
	    quiet=1
	    ;;
	"--version")
	    git_latexdiff_compute_version
            exit 0
	    ;;
	"--subtree")
	    subtree=1
	    ;;
	"--whole-tree")
	    subtree=0
	    ;;
	"--prepare")
	    shift
	    prepare_cmd="$1"
	    ;;
        "--latexmk")
            uselatexmk=1
            ;;
	"--latexpand")
	    shift
	    latexpand=$1
	    ;;
	"--bbl")
	    bbl=1
	    ;;
	"--latexdiff-flatten")
	    latexdiff_flatten=1
            flatten=0
	    ;;
	"--latexopt")
	    shift
	    latexopt=$1
	    ;;
        "--ln-untracked")
            ln_untracked=1
            ;;
        "--no-ln-untracked")
            ln_untracked=0
            ;;
        "--tmpdirprefix")
	    shift
	    tmpdir_prefix="$1"
	    ;;
        -*)
            if test "$1" = "--" ; then
                if test -z "$new" ; then
                    new=$1
                else
                    echo "Bad argument $1"
                    usage
                    exit 1
                fi
            else
                latexdiffopt+=("$1")
            fi
            ;;
        *)
	    if test -z "$1" ; then
		echo "Empty string not allowed as argument"
		usage
		exit 1
	    elif test -z "$old" ; then
		old=$1
	    elif test -z "$new" ; then
		new=$1
	    else
		echo "Bad argument $1"
		usage
		exit 1
	    fi
            ;;
    esac
    shift
done

if test -z "$new" ; then
    new=HEAD
fi
if test "$new" = "--"; then
    ln_untracked=1
fi

if test -z "$old" ; then
    echo "fatal: Please, provide at least one revision to diff with."
    usage
    exit 1
fi

if test -z "$PDFVIEWER" ; then
    verbose "Auto-detecting PDF viewer"
    candidates="xdg-open evince okular xpdf acroread"
    if test "$(uname)" = Darwin ; then
        # open exists on GNU/Linux, but does not open PDFs
	candidates="open $candidates"
    fi

    for command in $candidates; do
	if command -v "$command" >/dev/null 2>&1; then
	    PDFVIEWER="$command"
	    break
	else
	    verbose_progress
	fi
    done
    verbose_done "$PDFVIEWER"
fi

case "$view" in
    maybe|1)
	if test -z "$PDFVIEWER" ; then
	    echo "warning: could not find a PDF viewer on your system."
	    echo "warning: Please set \$PDFVIEWER or use --pdf-viewer CMD."
	    PDFVIEWER=false
	fi
	;;
esac

if test $flatten = 1 &&
    ! command -v latexpand 2>/dev/null; then
    echo "Warning: latexpand not found. Falling back to latexdiff --flatten."
    latexdiff_flatten=1
    flatten=0
fi

if test $latex = 1; then
    LATEX_EXEC=latex
else
    LATEX_EXEC=pdflatex
fi    

## end option parsing ##

check_knitr () {
    if test -z "$prepare_cmd"; then
	prepare_cmd="Rscript -e \"library(knitr); knit('$main')\""
    fi
    main="${main%\.*}.tex"
}

log_cmd () {
    log=$1
    shift
    if [ "$quiet" = 1 ]; then
	"$@" >$log 2>&1
    else
	"$@"
    fi
}

# main is relative to initial_dir (if returned)
if test -z "$main" ; then
    printf "%s" "No --main provided, trying to guess ... "
    main=$(git grep -l '^[ \t]*\\documentclass')
    # May return multiple results, but if so the result won't be a file.
    if test -r "$main" ; then
	echo "Using $main as the main file."
    else
	if test -z "$main" ; then
	    echo "No candidate for main file."
	else
	    echo "Multiple candidates for main file:"
	    printf "%s\n" "$main" | sed 's/^/\t/'
	fi
	die "Please, provide a main file with --main FILE.tex."
    fi
fi

ext=${main##*\.}
case "$ext" in
    Rnw) check_knitr ;;
    Rtex) check_knitr ;;
    *) ;;
esac

if test ! -r "$main" ; then
    die "Cannot read $main."
fi

verbose "Creating temporary directories"

git_prefix=$(git rev-parse --show-prefix)
git_dir="$(git rev-parse --git-dir)" || die "Not a git repository?"
cd "$(git rev-parse --show-cdup)" || die "Can't cd back to repository root"
git_dir=$(cd "$git_dir"; pwd)

# make main relative to git root directory
if test -n "$git_prefix" ; then
    main=$git_prefix$main
fi
mainbase=$(basename "$main" .tex)
maindir=$(dirname "$main")

tmpdir=$tmpdir_prefix/git-latexdiff.$$
mkdir "$tmpdir" || die "Cannot create temporary directory."

cd "$tmpdir" || die "Cannot cd to $tmpdir"

mkdir old new || die "Cannot create old and new directories."

verbose_done
verbose_say "Temporary directories: $tmpdir/old and $tmpdir/new"
verbose "Checking out old and new version"

cd old || die "Cannot cd to old/"
if test "$ln_untracked" = 1; then
    (
       mkdir -p "$maindir" && cd "$maindir" && ln -s "$initial_repo"/"$maindir"/* .
    )
fi

if test "$subtree" = 1; then
    checkoutroot=$git_prefix
else
    checkoutroot="."
fi

# Checkout a subtree, without touching the index ("git checkout" would)
(cd "$git_dir" && git archive --format=tar "$old" "$checkoutroot") | tar -xf -
verbose_progress
cd ../new || die "Cannot cd to new/"
if test "$ln_untracked" = 1; then
    (
       mkdir -p "$maindir" && cd "$maindir" && ln -s "$initial_repo"/"$maindir"/* .
    )
fi
if test "$new" != "--"; then
    # if new == "--" then diff working dir (already there thanks to ln
    # -s above).
    (cd "$git_dir" && git archive --format=tar "$new" "$checkoutroot") | tar -xf -
fi
verbose_progress
cd ..

verbose_done

for dir in old new
do
    verbose "Running preparation command $prepare_cmd in $dir/$git_prefix"
    ( cd "$dir/$git_prefix/" && log_cmd prepare.log eval "$prepare_cmd" )
    if test ! -f "$dir/$main"; then
	die "$prepare_cmd did not produce $dir/$main."
    fi
    verbose_done
done

# Option to use latexdiff --flatten instead of latexpand
if test "$latexdiff_flatten" = 1; then
    latexdiffopt+=("--flatten")
fi

# Shortcut to include bbl
if test "$bbl" = 1; then
    bblexpand=("--expand-bbl" "$mainbase.bbl")
else
    bblexpand=()
fi

# Create flattened documents and keep for debugging
if test "$flatten" = 1; then
    if [ "$bbl" = 1 ]; then
	if [ ! -f "old/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing old/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd old/"$maindir"
	    log_cmd pdflatex0.log pdflatex $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for old version"
	    fi
	fi
	if [ ! -f "new/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing new/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd new/"$maindir"
	    log_cmd pdflatex0.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for new version"
	    fi
	fi
    fi
    verbose "Running latexpand"
    (
	cd old/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > old-"$mainbase"-fl.tex \
	|| die "latexpand failed for old version"
    (
	cd new/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > new-"$mainbase"-fl.tex \
	|| die "latexpand failed for new version"
    verbose_done

    verbose "Running latexdiff ${latexdiffopt[*]} old-${mainbase}-fl.tex new-${mainbase}-fl.tex > ./diff.tex"
    latexdiff "${latexdiffopt[@]}" old-"$mainbase"-fl.tex new-"$mainbase"-fl.tex > diff.tex \
	|| die "latexdiff failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new-"$mainbase"-fl.tex new-"$mainbase"-fl.tex.orig
    mv -f diff.tex new/"$main"
    verbose_done
else
    verbose "Running latexdiff ${latexdiffopt[*]} old/$main new/$main > ./diff.tex"
    latexdiff "${latexdiffopt[@]}" old/"$main" new/"$main" > diff.tex \
	|| die "latexdiff failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new/"$main" new/"$main.orig"
    mv -f diff.tex new/"$main"
    verbose_done
fi

verbose "Compiling result"

compile_error=0
cd new/"$maindir" || die "Can't cd to new/$maindir"
if test -f Makefile && test "$ignoremake" != 1 ; then
    log_cmd make.log make || compile_error=1
elif test "$uselatexmk" = 1; then
    log_cmd latexmk.log latexmk -f -pdf -silent "$mainbase" || compile_error=1
else
    if [ "$ignorelatexerrors" = 1 ]; then
	latexopt="$latexopt -interaction=batchmode"
    elif [ "$quiet" = 1 ]; then
	latexopt="$latexopt -interaction=nonstopmode"
    else
	latexopt="$latexopt -interaction=errorstopmode"
    fi
    log_cmd pdflatex1.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    if test "$bibtex" = 1 ; then
	log_cmd bibtex.log bibtex "$mainbase" || compile_error=1
    fi
    if test "$biber" = 1 ; then
	log_cmd biber.log biber "$mainbase" || compile_error=1
    fi
    log_cmd pdflatex2.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    log_cmd pdflatex3.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
fi

verbose_done

if [ "$compile_error" = 1 ] && [ "$ignorelatexerrors" = 1 ]; then
    echo "LaTeX errors were found - but attempting to carry on."
    compile_error=0
fi

if test $latex = 1; then
    dvips "$mainbase".dvi
    ps2pdf "$mainbase".ps
fi

pdffile="$mainbase".pdf
if test ! -r "$pdffile" ; then
    echo "No PDF file generated."
    compile_error=1
fi

if test ! -s "$pdffile" ; then
    echo "PDF file generated is empty."
    compile_error=1
fi

if test "$compile_error" = "1" ; then
    echo "Error during compilation. Please examine and cleanup if needed:"
    echo "Directory: $tmpdir/new/$maindir"
    echo "     File: $mainbase.tex"
    # Don't clean up to let the user diagnose.
    exit 1
fi

if test -n "$output" ; then
    abs_pdffile="$PWD/$pdffile"
    (cd "$initial_dir" && mv "$abs_pdffile" "$output")
    echo "Output written on $output"
elif [ -f "$pdffile" ]; then
    new_pdffile="$tmpdir"/"$pdffile"
    mv "$pdffile" "$new_pdffile"
    pdffile="$new_pdffile"
fi


if test "$view" = 1  || test "$view" = maybe  && test -z "$output" ; then
    "$PDFVIEWER" "$pdffile"
fi

case "$cleanup" in
    "all")
	verbose "Cleaning-up result"
	cd ..
	cd ..
	rm -fr "$tmpdir"
	verbose_done
	;;
    "keeppdf")
	verbose "Cleaning-up all but pdf (kept in $pdffile)"
	rm -fr "$tmpdir"/old "$tmpdir"/new
	verbose_done
	;;
    "none")
	verbose_say "Generated files kept in $tmpdir/"
	;;
esac


==> scripts/style-check/common-typos <==
a the                % phrase double article
 pt                  % syntax ? I guess avoid straggling pt's that escape tex?
[ ],                 % syntax whitespace before comma seems wrong.
Figure Figure        % phrase pizza pizza.
[ ]-[ ]              % syntax a hyphen surrounded by space should probably be an emdash '---'
[0-9]-[0-9]          % syntax use an endash '--' for ranges
[0-9]ms              % syntax put a space between the number and the unit.
[^egs]\. [a-z]       % syntax a period usually ends a sentence, and sentences should start with a capital; doesn't apply for i.e.,
\.  [a-z]            % syntax a period usually ends a sentence, and sentences should start with a capital; "i.e." should have a comma following.
[a-z]\.\.            % syntax double period is rarely right, use \ldots for ellipsis
[^\\]"               % syntax use fancy quotes
\beg\.               % syntax should be e.g. as in "examples given"
from to\b            % phrase haven't used this properly.
help help            % phrase double word, that probably means the author paniced
of of                % phrase apparent double word.
the affect           % phrase should probably be 'the effect'
the the              % phrase apparent double word.
there too few        % phrase there are too few?
was not was          % phrase pretty much a joke if this gets matched.
we we                % phrase it would be oi oi in french, I guess.
with on              % phrase probably wrong.
with with            % phrase apparent double word.
[\n ]--[\n ]         % syntax that's an en-dash, you want an em-dash: "---"
my my                % phrase unlikely that's what you want, at least without a comma. (doesn't work across newlines)
>From                % syntax be careful when you email .tex files.  I've seen this slip through into submissions.
e\.t\.c\.            % syntax it's et cetera; use etc.
such as like         % phrase pick one
<<<<<<< .            % syntax CVS conflict!
=======              % syntax CVS conflict!
>>>>>>> [0-9]        % syntax CVS conflict!
e\.g\.[\n ]          % syntax should be followed with a comma, as e.g. can be read as "for example" (thanks JZ!)
i\.e\.[\n ]          % syntax should be followed with a comma, as i.e. can be read as "that is" (thanks JZ!)
[ ]\.[\n ]           % syntax stray period?
further more         % phrase one word: furthermore
safe guard           % phrase one word: safeguard
that be              % phrase mistake.
can not              % phrase cannot
only only            % phrase double word
is is                % phrase double word.
they shows           % phrase argh, mistake.
less that than       % phrase typo damage
from from            % phrase double word score
in in                % phrase "in" (common mistake)
not not              % phrase argh.
it it                % phrase argh.
to illicit           % phrase "to elicit" -- illicit is always an adjective.
c\.f\.               % phrase actually, it's cf., and you'd like cf.\ (backslash space)
this lead to         % phrase "led to" if past tense, "leads to" if present.
on on                % phrase double word.
has is               % phrase choose
description their    % phrase saw this, clearly wrong.
including:  % syntax I prefer no colon after including, which already says a list is coming.
[a-z]\([A-Z]  % syntax put a space before parens, even when introducing acronyms.
without and without % phrase saw this.
can be result       % phrase saw this typo.



==> scripts/style-check/foolish-phrases <==
(quite|more|very|most) unique    % phrase unique is.
(quite|more|very|most) abstract  % phrase abstract is.
tangible view                    % phrase mix that metaphor some more.
for e\.g\.                       % phrase e.g. includes "for".
begs the question                % phrase unless you're very clever: "raises the question": http://alt-usage-english.org/excerpts/fxbegthe.html
high rate of speed               % phrase local news-speak.
especially necessary             % phrase 'especially important', necessary may be an absolute like unique.
how will it effect % phrase you likely meant "affect"
how it will effect % phrase you likely meant "affect"
insure proper performance % phrase "ensure"
especially true                  % phrase 'especially important', true may be an absolute like unique.
to affect change                 % phrase "effect" change;  I read this on a poster.
higher results                   % phrase maybe higher performance or higher values.
is more general then the         % phrase probably "than"
upper bounding                   % phrase "limiting" or "setting an upper bound on"
in principal                     % phrase likely, "in principle"
literally like                   % phrase literally means no simile.  
design principal  % phrase likely, "design principle" 
different from 	    	   	 % phrase unlike

==> scripts/style-check/latex-checking <==
\{\\em [^\}]*[^\}\/]\}[:]    % syntax use \emph{} or explicit italic correction {\em foo\/}
\{\\em [^\}]*[:\.,]\}        % syntax punctuation at the edges of italic text is not italicized
[A-Z]{2,10}\.[ ]*[\n ][ ]*[A-Z]  % syntax intersentence spacing should be used if a sentence ends with an acronym: "FOO\\@."
\\etal[^{]                   % syntax it's good practice to use \etal{} to avoid bad spacing
\\caption\[[^\]]*[^\.]\]     % syntax short caption should end with a period.
\\caption\[.*CCDF.*\]        % syntax short caption should not include graph type.
\\caption\[.*CDF.*\]         % syntax short caption should not include graph type.
\\caption\[.{0,25}\]         % syntax short caption should not be too short.
th century                   % syntax use textsuperscript
[ ]---[ ]                    % syntax the em-dash should be right up against the words.
[ \n]---[ \n]                % syntax the em-dash should be right up against the words.
^---[ \n]                    % syntax the em-dash should be right up against the words.
[ \n]---$                    % syntax the em-dash should be right up against the words.
[ \n]--[ \n]                 % syntax the en-dash should be between numbers.
^--[ \n]                     % syntax the en-dash should be between numbers.
[ \n]--$                     % syntax the en-dash should be rbetween numbers.
,[~ ]\\etal                  % syntax no comma before etal (unless Smith, Martinez, \etal)
\\etal\{\}'s                 % syntax eew.
\\(sub)?section\{[A-Z][^}]*[ ][a-z]{5,40}[^}]*\} % syntax subsection headers should be initial capped.
\\(sub)?section\{[A-Z][^}]*[^:][ ]{1,}(With|A|An|Is|And|For|To|The)[ ][^}]*\} % syntax some words needn't be capitalized
[ ]\\footnote                % syntax no space before footnote.
\\footnote\{.*\}.            % syntax footnotes after punctuation
,,                           % syntax double comma is unlikely to be intentional.
cf\.[^\\]                    % phrase cf. should get an escaped space "\ "
et al\.[^\\]                    % phrase et al. should get an escaped space "\ "
[<>]  % syntax a less than or greater than outside math mode shows other characters.
in (section|table|figure) \\ref % phrase should have ~ before ref
section~\\ref % capitalize capitalize section when saying Section 6.
table~\\ref % capitalize capitalize section when saying Table 6.
figure~\\ref % capitalize capitalize section when saying Figure 6.
\\(sub)?section\{Intro\} % syntax spell it out.
,''                          % syntax punctuation outside quotes
\.\.\.                       % syntax use \dots

==> scripts/style-check/my-rules <==
#  such may be abused to blacklist certain words even spelled correctly.
# capitalize is case sensitive, and also bracketed by non-word.
# phrase and spelling are case insensitive, but bracketed by non-word characters.
# syntax is case sensitive but not bracketed by non-word; probably best if used with regexes.
\bet al\.[^}]        % syntax use the \etal{} command instead. (or write one to italicize)
\bet\. al\.          % syntax use the \etal{} command, "et" needs no dot (et alii). (or write one to italicize)
\bc\.f\.\b             % syntax should be cf. for "confer" (latin for compare)
\b$i\)[^$]              % syntax leave the paren in math mode -- should be $i)$
\b$ii\)[^$]             % syntax leave the paren in math mode -- should be $ii)$
\b$iii\)[^$]            % syntax leave the paren in math mode -- should be $iii)$
\b$iv\)[^$]             % syntax leave the paren in math mode -- should be $iv)$
\b$v\)[^$]              % syntax leave the paren in math mode -- should be $v)$
\ban [b-df-gj-np-tv-z] % syntax probably meant to use "a" instead of "an", though there are exceptions.
\ban [B-DF-GJ-NP-TV-Z][^A-Z/] % syntax probably meant to use "a" instead of "an", though there are exceptions (like acronyms).
\b[Aa] [aeiouAEIOU](?!se|ni|A|ur|RL|ti|ne|DP) % syntax probably meant to use "an" instead of "a", though there are exceptions. (user, useful, AA, unified, uniform, unique, Europe, one, UDP; n/a doesn't work, so use {n/a})
This allows           % phrase tie more explicitly: This (x) allows...
we find               % phrase omit "we find"
we found              % phrase omit "we found"
try and               % phrase "try to", though if you're using try as a noun in a compound sentence, this rule is wrong.
impact of             % phrase not a useful metaphor; try evaluation, success, effect, value.
including [^\.]*etc\. % syntax "including" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
includes [^\.]*etc\.  % syntax "includes" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
and etc\.             % phrase come on. learn some latin.
AT&T                  % syntax you poor thing, this won't compile.
doesn't               % phrase be formal.
be occur              % phrase what happens when I'm indecisive about what follows "can"
up until              % phrase "until"
one or more           % phrase probably redundant -- nonzero is probably implied.
is comprise(d|s) of   % phrase you probably mean "is composed of" because "comprises" is more a synonym for "contains" 
will be significantly different % phrase "will differ significantly" for active voice
More importantly,     % phrase probably means the order is wrong: put important stuff first.
todo                  % ignoredcommand
texttt                  % ignoredcommand
jbgcomment              % ignoredcommand
lkfcomment              % ignoredcommand
due to space constraints % phrase don't whine.
this paper % phrase can be ambiguous if talking about someone else's paper whether you mean the one youre writing or the one you're talking about..
the above             % phrase horrible phrase that must be expunged.  you might use "these" instead, but best to make the sentence stand alone.
referred to above     % phrase "these".
(all|the|of) [0-9][ ] %  phrase use words for numbers in phrases.
clearly shows         % phrase "clearly" is usually much.
grows larger          % phrase is "grows smaller" possible?  grows.
guarantee as much as possible % phrase then not really a guarantee "provide"
affects negatively   % phrase "hurts" or "harms"
rely upon % phrase rely on is good enough
relies upon % phrase relies on is good enough
record route packets? % phrase hyphenate record-route packets
record-route; % phrase leave record route alone if not modifying something else
we accomplish this  % phrase verbose way to get active voice.
refers to the % phrase you're being wimpy in the definition.  use "is"
\\emph\{[a-zA-Z ]*\} refers to % syntax you're being wimpy in the definition.
loss off % phrase loss of?
this could % phrase this "what" could
with that has % phrase probably just one
simply % phrase probably isn't.
to get to % phrase "to reach"?
latency benefit % phrase reduction
latency improvement % phrase reduction
shed insight % phrase 'shed light' would seem the metaphor.
increasingly more % phrase redundant
I\.e\. % syntax starting a sentence with i.e. is just ugly.
E\.g\. % syntax starting a sentence with e.g. is just ugly.
in the large % phrase if large is a noun, bad.  if it's an adjective, fine.
encapsulates with % phrase seen it, don't know what it means.
when working with % phrase just say "with"
it is true that	  % phrase usually can delete
LDA % phrase convention put in small caps
(F|f)indings (show|indicate|suggest)	% phrase delete or make more specific

==> scripts/style-check/networking-research <==
IPs                  % phrase should be IP addresses
[Rr]ate-limits       % spelling "rate limits" has no hyphen, only "rate-limited"
best effort          % phrase hyphenate best-effort service.
deliver route        % phrase jargon redundancy
euclidean % capitalize Euclidean.
interdomain          % spelling inter-domain
internet             % capitalize unless talking about an internet other than the Internet
intradomain          % spelling intra-domain
log-normal           % spelling lognormal is one word.
pareto               % capitalize
ttl                  % capitalize
weibull              % capitalize proper name.
PoP                  % syntax I think POP looks less annoying.
PoPs                 % syntax I think POP looks less annoying.
http[ ]              % capitalize capitalize HTTP.
linux                % capitalize capitalize Linux
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
zipf                 % capitalize capitalize the guy's name.


==> scripts/style-check/passive-voice <==
it is possible to                   % phrase passive voice, try: "can"
are identified by                   % phrase passive
is shown                            % phrase passive.
is not included in                  % phrase maybe this is passive
there (are|is) [^\.:;]* (that|in)   % phrase maybe this is passive
can be evaluated                    % phrase avoid passive: I evaluated
can be observed                     % phrase avoid passive: are visible
# is needed                         % phrase passive voice
is used to                          % phrase go active voice, or subsititute "helps"
(are|were) needed[^\?]              % phrase passive voice
(is|are) presented in               % phrase "appears in", or reword to avoid passive voice
it is possible that                 % phrase "may"
(is|are) (depicted|illustrated|sketched) in  % phrase thats passive voice
(is|are) shown in                   % phrase "shows"
as can be seen in                   % phrase X shows that Y.
there needs to be                   % phrase passive voice in a bad way.
was designed                        % phrase passive voce.
it may be                           % phrase passive "it"
it is important that                % phrase passive; replace with X is important because Y.


==> scripts/style-check/verbose-phrases <==
a large number of                   % phrase you mean "many"
a substantial number of             % phrase how substantial?  most?  or just enough that can't be ignored?
an insufficient number of           % phrase "too few"
a significant number of             % phrase one is significant.   consider "prohibitive" if the number is sufficient to be problematic.
a number of                         % phrase getting the verb agreement for this useless phrase is tricky.
a number of different               % phrase use "different" (should have a high score)
a small number of                   % phrase you mean "few"
a low number of                   % phrase you mean "few"
a relatively low number of                   % phrase you mean "few"
actually                            % spelling probably doesn't add
to an extent                        % phrase you can probably remove
and instead                         % phrase replace with but?
be done                             % phrase if "X of Y can be done", try "Y can be Xed"; it's already passive voice.
combining multiple                  % phrase as opposed to "combining one?"
aggregating multiple                % phrase "aggregating"
do this                             % phrase probably verbose if you use a pronoun for what you're doing
exists[ ]                           % phrase probably no better than "is", but end of sentence may be unavoidable?
if it is to                         % phrase should be "to" (usually followed by "be X")
if they are to                      % phrase should be "to" (usually followed by "be X")
in general                          % phrase unless matched with "in specific," this is usually useless; perhaps "overall"
in order to                         % phrase remove "in order" and get "to"
in the past                         % phrase past tense is likely enough.
in the way of                       % phrase should be "as"
counting the number of              % phrase counting.  dude.
is permitted to                     % phrase "may"
largely opaque                      % phrase largely does not modify opaque
makes a new                         % phrase should be "creates"
may not chose                       % phrase "may not" is future tense; "chose" is past.
one should note                     % phrase just write it.
note that                           % phrase is the rest of the paper less notable?
Note, that                          % syntax not only should you not "note that", no comma after note.
we note                             % phrase is the rest of the paper less notable?
note however that                   % phrase is the rest of the paper less notable?
it is important to note             % phrase is the rest of the paper less notable?
really                              % phrase probably doesn't add; if you think it does, use "r{}eally" -- don't change to 'in fact'
in fact				    % phrase cut
rigorously                          % spelling probably doesn't add, and I rarely do anything with rigor
the way in which                    % phrase should be "how" or ""
the manner in which                 % phrase should be "how" or ""
value stems                         % phrase value is derived or offered, I think.
time at which                       % phrase very likely "when"
place at which                      % phrase very likely "where"
at the time                         % phrase very likely "when"
reduced number of                   % phrase very likely "fewer" or maybe maybe "less"
is present in                       % phrase present is probably redudant, try "is in"
they all                            % phrase maybe "all xs" would be better.
easy to do                          % phrase "feasible" or "practical" might be better.
is going to                         % phrase "will".
are going to                        % phrase "will".
getting                             % phrase probably "receiving" or "querying"
those are                           % phrase see if "those X are" is clearer?
design is motivated                 % phrase "inspired by" is probably better than "motivated" for design
locations throughout the world      % phrase drop "throughout the world"
e.g., as opposed to                 % phrase if you're giving examples, you're not talking about what isn't.  drop "e.g."
in addition, we also                % phrase remove either "also" or "in addition"
other related issues                % phrase probably remove "other"
the aforementioned                  % phrase "these xs" or "this x" would be less snooty
center around                       % phrase (cook) a center is a point: "center on" is okay.
could care less                     % phrase (cook) 'really? how much less could you care?' (should be couldn't)
grouped together                    % phrase redundant.  "grouped" alone should suffice.
put together                        % phrase long: "construct" "build" or "assemble"
consistent with each other          % phrase redundant.  "consistent" suffices.
be accomplished with                % phrase try "requires" "uses" "needs"?
the lack of knowledge of            % phrase would "X is unknown" work better?
gets to know                        % phrase you mean "learns"
trying to look like                 % phrase you mean "acting", "emulating", or "mimicing"
has got to be                       % phrase "must be"
got                                 % phrase try "became" "received" ?
gotten                              % phrase try "helped" ?
live in a vacuum                    % phrase a tired metaphor that makes me want to vomit.
positive impact                     % phrase try "benefit"
negative impact                     % phrase try "harm" or "consequences"
adverse impact                      % phrase try "harm" or "consequences"
adversely impacting                 % phrase try "harming" or "hurting"
discuss the issues of               % phrase could probably drop "the issues of" unless there's a list
the presence of                     % phrase not far from 'is', 'has', etc.
does not allow                      % phrase consider "forbids" or "prohibits"
and/or                              % phrase just say or.
there is the potential to           % phrase just say may.
there is the possibility that       % phrase just say might.
can be achieved                     % phrase maybe not so good?
find out                            % phrase perhaps determine?
in the absence of                   % phrase perhaps without?
in the presence of                  % phrase perhaps with?
set up                              % phrase perhaps create, configure, or initialize
in the face of                      % phrase can be overused.  try despite?
several times (at|of)               % phrase discouraged by Kurt.
a large degree of                   % phrase ick.
we start by first                   % phrase redundant. ("first, we" or "we start by").
in general, they are usually        % phrase redundant.
refers to the notion                % phrase define your term precisely if possible.
a significant amount of             % phrase probably just "significant"
real practical                      % phrase as opposed to imaginary practical?
people that are                     % phrase use people who are?
additional detail that we add       % phrase as opposed to additional detail that we subtract?
in some cases and not in others     % phrase "in some cases"
it is known that                    % phrase just say it.
caused due to                       % phrase "caused by"
a result of the fact that           % phrase "caused by"
results (indicate|show|suggest)     % phrase drop
research (indicates|show|suggest)   % phrase drop
can be attributed to the fact that  % phrase "is because"
a large set of                      % phrase probably don't care that it is a set.
a small set of                      % phrase probably don't care that it is a set: use 'a few'
provides a look at                  % phrase (timid) probably mean "shows".
in most cases                       % phrase "usually"
continue into the forseeable future % phrase "continue".
for the forseeable future           % phrase drop.
fail to successfully                % phrase "fail to" is sufficient.
Clearly,                            % syntax starting a sentence with clearly confuses me.
in different continents             % phrase ON different continents, IN different countries
(we|to) handle                      % phrase use a more specific verb like address, treat, solve
handling                            % phrase use a more specific verb like addressing, treating, solving, mitigating (unless handling errors or exceptions)
For the purposes of                 % phrase "For"
We observe that                     % phrase drop.
some degree of                      % phrase "some"
in the problem of                   % phrase (contributed by rap)
conclude several things             % phrase make (draw) several conclusions
extra bonus                         % phrase "bonus"
added bonus                         % phrase "bonus"
it is important to emphasize that   % phrase use diction to emphasize.
it is possible that                 % phrase "x may y"
caused due to                       % phrase "caused by"
recent work by                      % phrase could maybe be dropped, as the cite will include the date.
identify the location of            % phrase "find"
that go across                      % phrase "that cross"
ideally, we would like              % phrase "we would like"
enabling the ability to             % phrase "supporting" or "allowing" or "permitting"
absolutely essential                % phrase essential is.
we essentially do                   % phrase essentially is a poor adverb.  "The essence of our algorithm is a..."
Essentially,                        % phrase maybe "In essence," but could also be removed.
In this section (we|I)              % phrase "In this section, we", or "In this section, I"
essentially all                     % phrase "most"
past experience                     % phrase "experience" http://www.cmu.edu/styleguide/trickywords.html
particulary difficult primarily     % phrase simplify
intuition about why                 % phrase "intuition as to why"
Recall from above                   % phrase "recall"
Further, (I|we) will also           % phrase drop further or also
respectively                        % phrase unneeded.
in terms of                         % phrase don't need this.
the extent to which                 % phrase "how much"
make sure                           % phrase "ensure"
make up                             % phrase "constitute" "compose"
make use of                         % phrase "use"
make a decision                     % phrase "decide"
make a guess                        % phrase "guess"
since that time                     % phrase "since then"
choices to make                     % phrase "choices"
certain limitations                 % phrase what does 'certain' add to limitations?
will [a-z]* in the future           % phrase "will"
business entities                   % phrase "businesses"
rely primarily on                   % phrase "primarily" weakens "rely".  perhaps just "use" would be simpler.
has the potential to                % phrase can
have not yet developed              % phrase "have yet to develop"
to be effective,                    % phrase probably redundant.
provide information about           % phrase "tell how" "reveal" "expose" "disclose"
are different,                      % phrase "differ"
have already been                   % phrase "have been"? "were"?
as appropriate                      % phrase not needed?
only rarely                         % phrase "rarely" is probably enough.
is effective at                     % phrase "can"
foremost among them is              % phrase "foremost is" would be shorter.
those that have no                  % phrase those without
that have no                        % phrase "without"?
a variety of diverse                % phrase redundant
be highly valuable in               % phrase simplify.
the overall goal                    % phrase 'the goal'
sometimes an? [a-z]+ will           % phrase an x may
this is perhaps because             % phrase this may be because
adding an additional                % phrase redundant
IP protocol                         % phrase redundant
works well                          % phrase be more specific.
something                           % phrase could eliminate.
to keep from                        % phrase "to avoid"
[\.,] since (!then)                 % phrase probably you mean "because" unless you're talking about time. -- "has since" is okay.
performance characteristics         % phrase rare that characteristics adds.
takes into account                  % phrase considers
specify particular                  % phrase if specifying, particular should be redundant.
prototype implementation            % phrase "implementation" is redundant.
given a particular                  % phrase "given a" is probably enough
described in detail (in|below)      % phrase use "detailed"
relatively more                     % phrase more is already relative.
focus primarily on                  % phrase bad metaphor: subject of focus is singular.
primary focus                       % phrase bad metaphor: subject of focus is singular.
relatively more                     % phrase more is already relative.
gives [a-z]+ [a-z]+ information about % phrase use "tells" x
gives [a-z]+ information about      % phrase use "tells" x
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
have an effect on                   % phrase "affect"
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
we can see                          % phrase "we can see" isn't formal enough.
still remain                        % phrase "remain".
change over time                    % phrase "change"
turn into                           % phrase "become"
looking back in retrospect          % phrase pick.
ensures that there will be no       % phrase "prevents"
does have                           % phrase "has"
first step toward this              % phrase "toward this" can probably be dropped.
can potentially be                  % phrase "might be", or just "can be"
obviates the need for               % phrase just obviates x, not obviates the need for x.
it is indeed                        % phrase "it is", though still passive.
planning in advance                 % phrase when else might you plan?
a lot of                            % phrase "many"
keep in mind                        % phrase "consider" (or drop)
it is clear that                    % phrase if clear, you don't have to say it.
especially true                     % phrase true is an absolute, can't be especially true.
making it increasingly difficult    % phrase preventing, discouraging, impeding, blocking, slowing...
is potentially                      % phrase "may be"
have been [a-z]* in the past        % phrase 'in the past' is redundant with tense.
amount of time  % phrase "duration"
should ideally % phrase "should"
are of great benefit to % phrase "help" or "aid"
are of benefit to % phrase "help" or "aid" or "promote"
important here % phrase consider "relevant"
while at the same time % phrase "while" is enough.
are able to % phrase can
subvert the proper operation of % phrase subvert
speed slow % phrase speed is probably redundant.
of size no smaller than % phrase "of size" is probably redundant
of size no larger than % phrase "of size" is probably redundant
of size smaller than % phrase "of size" is probably redundant
of size larger than % phrase "of size" is probably redundant
might potentially % phrase "might"
in the context of % phrase "in" avoid, if possible.
increase the amount of % phrase probably just increase.
show the difference between % phrase compare
in addition, we also % phrase pick.
overhead efficiency % phrase huh?
have an effect on % phrase "affect"
have a signficant effect on %  phrase "affect"
we find % phrase can usually be removed
this suggests % phrase remove or make more precise
effective for providing	   	 % phrase remove
we performed a                   % phrase just use the verb directly
we perform a                     % phrase just use the verb directly
were able to                     % phrase could
are able to                      % phrase can

